Bayesian grey-box identification of nonlinear convection effects in heat transfer dynamics

We propose a computational procedure for identifying convection in heat transfer dynamics. The procedure is based on a Gaussian process latent force model, consisting of a white-box component (i.e., known physics) for the conduction and linear convection effects and a Gaussian process that acts as a black-box component for the nonlinear convection effects. States are inferred through Bayesian smoothing and we obtain approximate posterior distributions for the kernel covariance function's hyperparameters using Laplace's method. The nonlinear convection function is recovered from the Gaussian process states using a Bayesian regression model. We validate the procedure by simulation error using the identified nonlinear convection function, on both data from a simulated system and measurements from a physical assembly.

==> preambles/math-notation.tex <==

\renewcommand{\d}[1]{\operatorname{d}\!{#1}} % integration term
\renewcommand{\exp}[1]{\operatorname{exp}\!\left({#1}\right)}
\renewcommand{\log}[1]{\operatorname{log}\!\left({#1}\right)}
\newcommand{\lognb}[1]{\operatorname{log}{#1}} % log without brackets
\renewcommand{\ln}[1]{\operatorname{ln}\!\left({#1}\right)}
\newcommand{\tr}[1]{\operatorname{tr}\!\left({#1}\right)} % trace
\newcommand{\argmax}[2]{\underset{#1}{\operatorname{argmax}}\!\left({#2}\right)}
\newcommand{\mean}[1]{\bar{#1}} % mean as overbar
\newcommand{\cov}[1]{\mathbf{S}_{#1}} % covariance matrix
\newcommand{\covs}[1]{S_{#1}} % covariance for 1d
\newcommand{\T}{\operatorname{T}} % transpose
\newcommand{\vect}[1]{\boldsymbol{#1}} % vector as bold
\newcommand{\matr}[1]{\mathbf{#1}} % matrix as bold capital
\newcommand{\E}[1]{\mathbb{E}\!\left[{#1}\right]} % expectation
\newcommand{\U}[1]{\mathbb{U}\!\left[{#1}\right]} % average energy
\newcommand{\Ux}[2]{\mathbb{U}_{#1}\!\left[{#2}\right]} % average energy with respect to a variable
\renewcommand{\H}[1]{\mathbb{H}\!\left[{#1}\right]} % entropy
\newcommand{\Hx}[2]{\mathbb{H}_{#1}\!\left[{#2}\right]}
\newcommand{\F}[1]{\operatorname{F}\!\left[{#1}\right]} % free energy
\newcommand{\Fx}[2]{\operatorname{F}_{#1}\!\left[{#2}\right]}
\newcommand{\Ex}[2]{\mathbb{E}_{#1}\!\left[{#2}\right]} % expectation with respect to a specific term
\newcommand{\Exm}[2]{\underset{#1}{\mathbb{E}}\!\left[{#2}\right]} % expectation with respect to many terms, denoted below the operator
\newcommand{\Etx}[2]{\tilde{\mathbb{E}}_{#1}\!\left[{#2}\right]}
\newcommand{\Var}[1]{\mathbb{V}\!\operatorname{ar}\!\left[{#1}\right]}
\newcommand{\Cov}[1]{\mathbb{C}\!\operatorname{ov}\!\left[{#1}\right]}
\newcommand{\Covx}[2]{\mathbb{C}\!\operatorname{ov}_{#1}\!\left[{#2}\right]}
\newcommand{\N}[1]{\mathcal{N}\!\left({#1}\right)}
\newcommand{\MN}[1]{\mathcal{MN}\!\left({#1}\right)}
\newcommand{\W}[1]{\mathcal{W}\!\left({#1}\right)}
\newcommand{\logN}[1]{\operatorname{log}\!\mathcal{N}\!\left({#1}\right)}
\newcommand{\Gam}[1]{\mathcal{G}am\!\left({#1}\right)}
\newcommand{\Bern}[1]{\mathcal{B}ern\!\left({#1}\right)}
\newcommand{\Cat}[1]{\mathcal{C}at\!\left({#1}\right)}
\newcommand{\Con}[1]{\mathcal{C}on\!\left({#1}\right)}
\newcommand{\Beta}[1]{\mathcal{B}eta\!\left({#1}\right)}
\newcommand{\Dir}[1]{\mathcal{D}ir\!\left({#1}\right)}
\newcommand{\Exp}[1]{\mathcal{E}xp\!\left({#1}\right)}
\newcommand{\Ig}[1]{\mathcal{I}g\!\left({#1}\right)}
\newcommand{\Uni}[1]{\mathcal{U}\!\left({#1}\right)}
\newcommand{\logb}[2]{\operatorname{log}_{#1}\!\left({#2}\right)} % log with specific base

\newcommand\yestag{\addtocounter{equation}{1}\tag{\theequation}} % the opposite of notag, e.g. for use in a align* environment

\def\bfy{\mathbf{y}}
\def\bfx{\mathbf{x}}
\def\bfu{\mathbf{u}}
\def\sfy{\mathsf{y}}
\def\sfx{\mathsf{x}}
\def\sfu{\mathsf{u}}
\def\rmd{\mathrm{d}}
\def\cN{\mathcal{N}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cJ{\mathcal{J}}
\def\-{\text{-}}
\def\+{\text{+}}
\def\tr{\text{tr}}
\newcommand\given[1][]{\:#1\vert\:}
\newcommand\euler{\textit{e}}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newcommand{\HRule}[1]{\rule{\linewidth}{#1}}

==> preambles/tikz.tex <==
% Preamble for drawing FFGs. For example:

% \begin{tikzpicture}
%     [node distance=20mm,auto,>=stealth']
%     \begin{scope}
%         %\draw[style=dotted] (0,-10cm) grid[xstep=1cm, ystep=1cm] (12cm,6cm);

%         \node[clamped] (fl) {};
%         \node[box, right of=fl, node distance=15mm] (fa) {$f_a$};
%         \node[box, right of=fa] (fb) {$f_b$};
%         \node[box, right of=fb] (fc) {$f_c$};
%         \node[clamped, right of=fc, node distance=15mm] (fr) {};
%         \node[clamped, below of=fb, node distance=15mm] (fd) {};

%         \path[line] (fl) edge[-] node[anchor=north]{$x_1$} (fa);
%         \path[line] (fa) edge[-] node[anchor=north]{$x_2$} (fb);
%         \path[line] (fb) edge[-] node[anchor=north]{$x_5$} (fc);
%         \path[line] (fc) edge[-] node[anchor=north]{$x_4$} (fr);
%         \path[line] (fb) edge[-] node[anchor=west]{$x_3$} (fd);

%         \msg{up}{right}{fa}{fb}{0.5}{1}
%         \msg{up}{right}{fb}{fc}{0.35}{2}
%         \msg{up}{left}{fb}{fc}{0.65}{3}
%     \end{scope}    
% \end{tikzpicture}

\usepackage{tikz}
\usepackage{xifthen}

\pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main}  % set the order of the layers (main is the standard layer)
\definecolor{beige}{RGB}{245, 245, 220}
\definecolor{darkgrey}{RGB}{75, 75, 75}
\definecolor{lightgrey}{RGB}{250, 250, 250}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}
\newcommand*\smallcircled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0pt,minimum width=3.5mm] (char) {#1};}}

\usetikzlibrary{calc, arrows, fit, positioning, patterns, decorations.pathreplacing, shapes}
\tikzstyle{dash} = [dashed, -latex,>=latex]
\tikzstyle{line} = [draw, -latex,>=latex]
\tikzstyle{box} = [draw, minimum size=.8cm]
\tikzstyle{roundbox} = [draw, circle, inner sep=0pt, minimum size=3mm]
\tikzstyle{clamped} = [draw, fill=black, minimum size=0.15cm]
\tikzstyle{msgcircle} = [shape=circle, draw, inner sep=0pt, minimum size=5mm, fill=white]
\tikzstyle{darkmsgcircle} = [shape=circle, draw, inner sep=0pt, minimum size=5mm, fill=darkgrey, text=white, font=\bfseries]
\tikzstyle{msgdoublecircle} = [shape=circle, double, double distance=1.5pt, draw, inner sep=0pt, minimum size=5mm, fill=white]
\tikzstyle{darkmsgdoublecircle} = [shape=circle, double, double distance=1.5pt, draw, inner sep=0pt, minimum size=5mm, fill=darkgrey, text=white, font=\bfseries]

% Plate notation argument order: x-left, x-right, y-top, y-bottom
\newcommand{\brackets}[4]{
	\draw[dotted, rounded corners=0.3cm, line width = 1pt] ($({#1},{#3})+(-0.3,0)$) -- ($({#1},{#3})+(-0.3,0.3)$) -- ($({#2},{#3})+(0.3,0.3)$) -- ($({#2},{#3})+(0.3,0)$);
	\draw[dotted, rounded corners=0.3cm, line width = 1pt] ($({#1},{#4})+(-0.3,0)$) -- ($({#1},{#4})+(-0.3,-0.3)$) -- ($({#2},{#4})+(0.3,-0.3)$) -- ($({#2},{#4})+(0.3,0)$);}

% Message notation argument order:
%     Circle position relative to arrow [up, down, left, right];
%     Arrow direction [up, down, left, right];
%     Start node coordinate;
%     End node coordinate
%     Position along edge;
%     Message text;
\newcommand{\msg}[6]{
      % Circle left arrow down
      \ifthenelse{\isin{#1}{left} \AND \isin{#2}{down}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgcircle, xshift=-5.5mm] at (anchor) {#6};
            \node[xshift=-1.5mm] at (anchor) {$\downarrow$};
      }{}
      % Circle right arrow down
      \ifthenelse{\isin{#1}{right} \AND \isin{#2}{down}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgcircle, xshift=5.5mm] at (anchor) {#6};
            \node[xshift=1.5mm] at (anchor) {$\downarrow$};
      }{}

      % Circle down arrow right
      \ifthenelse{\isin{#1}{down} \AND \isin{#2}{right}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgcircle, yshift=-6.0mm] at (anchor) {#6};
            \node[yshift=-2.0mm] at (anchor) {$\rightarrow$};
      }{}
      % Circle up arrow right
      \ifthenelse{\isin{#1}{up} \AND \isin{#2}{right}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgcircle, yshift=6.0mm] at (anchor) {#6};
            \node[yshift=2.0mm] at (anchor) {$\rightarrow$};
      }{}

      % Circle down arrow left
      \ifthenelse{\isin{#1}{down} \AND \isin{#2}{left}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgcircle, yshift=-6.0mm] at (anchor) {#6};
            \node[yshift=-2.0mm] at (anchor) {$\leftarrow$};
      }{}
      % Circle up arrow left
      \ifthenelse{\isin{#1}{up} \AND \isin{#2}{left}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgcircle, yshift=6.0mm] at (anchor) {#6};
            \node[yshift=2.0mm] at (anchor) {$\leftarrow$};
      }{}

      % Circle left arrow down
      \ifthenelse{\isin{#1}{left} \AND \isin{#2}{up}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgcircle, xshift=-5.5mm] at (anchor) {#6};
            \node[xshift=-1.5mm] at (anchor) {$\uparrow$};
      }{}
      % Circle right arrow down
      \ifthenelse{\isin{#1}{right} \AND \isin{#2}{up}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgcircle, xshift=5.5mm] at (anchor) {#6};
            \node[xshift=1.5mm] at (anchor) {$\uparrow$};
      }{}
}

% Dark messages
\newcommand{\darkmsg}[6]{
      % Circle left arrow down
      \ifthenelse{\isin{#1}{left} \AND \isin{#2}{down}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[darkmsgcircle, xshift=-5.5mm] at (anchor) {#6};
            \node[xshift=-1.5mm] at (anchor) {$\downarrow$};
      }{}
      % Circle right arrow down
      \ifthenelse{\isin{#1}{right} \AND \isin{#2}{down}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[darkmsgcircle, xshift=5.5mm] at (anchor) {#6};
            \node[xshift=1.5mm] at (anchor) {$\downarrow$};
      }{}

      % Circle down arrow right
      \ifthenelse{\isin{#1}{down} \AND \isin{#2}{right}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[darkmsgcircle, yshift=-6.0mm] at (anchor) {#6};
            \node[yshift=-2.0mm] at (anchor) {$\rightarrow$};
      }{}
      % Circle up arrow right
      \ifthenelse{\isin{#1}{up} \AND \isin{#2}{right}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[darkmsgcircle, yshift=6.0mm] at (anchor) {#6};
            \node[yshift=2.0mm] at (anchor) {$\rightarrow$};
      }{}

      % Circle down arrow left
      \ifthenelse{\isin{#1}{down} \AND \isin{#2}{left}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[darkmsgcircle, yshift=-6.0mm] at (anchor) {#6};
            \node[yshift=-2.0mm] at (anchor) {$\leftarrow$};
      }{}
      % Circle up arrow left
      \ifthenelse{\isin{#1}{up} \AND \isin{#2}{left}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[darkmsgcircle, yshift=6.0mm] at (anchor) {#6};
            \node[yshift=2.0mm] at (anchor) {$\leftarrow$};
      }{}

      % Circle left arrow down
      \ifthenelse{\isin{#1}{left} \AND \isin{#2}{up}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[darkmsgcircle, xshift=-5.5mm] at (anchor) {#6};
            \node[xshift=-1.5mm] at (anchor) {$\uparrow$};
      }{}
      % Circle right arrow down
      \ifthenelse{\isin{#1}{right} \AND \isin{#2}{up}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[darkmsgcircle, xshift=5.5mm] at (anchor) {#6};
            \node[xshift=1.5mm] at (anchor) {$\uparrow$};
      }{}
}

\newcommand{\bwmsg}[6]{
      % doublecircle left arrow down
      \ifthenelse{\isin{#1}{left} \AND \isin{#2}{down}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgdoublecircle, xshift=-5.5mm] at (anchor) {#6};
            \node[xshift=-1.5mm] at (anchor) {$\downarrow$};
      }{}
      % doublecircle right arrow down
      \ifthenelse{\isin{#1}{right} \AND \isin{#2}{down}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgdoublecircle, xshift=5.5mm] at (anchor) {#6};
            \node[xshift=1.5mm] at (anchor) {$\downarrow$};
      }{}

      % doublecircle down arrow right
      \ifthenelse{\isin{#1}{down} \AND \isin{#2}{right}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgdoublecircle, yshift=-6.0mm] at (anchor) {#6};
            \node[yshift=-2.0mm] at (anchor) {$\rightarrow$};
      }{}
      % doublecircle up arrow right
      \ifthenelse{\isin{#1}{up} \AND \isin{#2}{right}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgdoublecircle, yshift=6.0mm] at (anchor) {#6};
            \node[yshift=2.0mm] at (anchor) {$\rightarrow$};
      }{}

      % doublecircle down arrow left
      \ifthenelse{\isin{#1}{down} \AND \isin{#2}{left}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgdoublecircle, yshift=-6.0mm] at (anchor) {#6};
            \node[yshift=-2.0mm] at (anchor) {$\leftarrow$};
      }{}
      % doublecircle up arrow left
      \ifthenelse{\isin{#1}{up} \AND \isin{#2}{left}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgdoublecircle, yshift=6.0mm] at (anchor) {#6};
            \node[yshift=2.0mm] at (anchor) {$\leftarrow$};
      }{}

      % doublecircle left arrow down
      \ifthenelse{\isin{#1}{left} \AND \isin{#2}{up}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgdoublecircle, xshift=-5.5mm] at (anchor) {#6};
            \node[xshift=-1.5mm] at (anchor) {$\uparrow$};
      }{}
      % doublecircle right arrow down
      \ifthenelse{\isin{#1}{right} \AND \isin{#2}{up}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgdoublecircle, xshift=5.5mm] at (anchor) {#6};
            \node[xshift=1.5mm] at (anchor) {$\uparrow$};
      }{}
}

% Dark messages
\newcommand{\bwdarkmsg}[6]{
      % doublecircle left arrow down
      \ifthenelse{\isin{#1}{left} \AND \isin{#2}{down}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[darkmsgdoublecircle, xshift=-5.5mm] at (anchor) {#6};
            \node[xshift=-1.5mm] at (anchor) {$\downarrow$};
      }{}
      % doublecircle right arrow down
      \ifthenelse{\isin{#1}{right} \AND \isin{#2}{down}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[darkmsgdoublecircle, xshift=5.5mm] at (anchor) {#6};
            \node[xshift=1.5mm] at (anchor) {$\downarrow$};
      }{}

      % doublecircle down arrow right
      \ifthenelse{\isin{#1}{down} \AND \isin{#2}{right}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[darkmsgdoublecircle, yshift=-6.0mm] at (anchor) {#6};
            \node[yshift=-2.0mm] at (anchor) {$\rightarrow$};
      }{}
      % doublecircle up arrow right
      \ifthenelse{\isin{#1}{up} \AND \isin{#2}{right}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[darkmsgdoublecircle, yshift=6.0mm] at (anchor) {#6};
            \node[yshift=2.0mm] at (anchor) {$\rightarrow$};
      }{}

      % doublecircle down arrow left
      \ifthenelse{\isin{#1}{down} \AND \isin{#2}{left}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[darkmsgdoublecircle, yshift=-6.0mm] at (anchor) {#6};
            \node[yshift=-2.0mm] at (anchor) {$\leftarrow$};
      }{}
      % doublecircle up arrow left
      \ifthenelse{\isin{#1}{up} \AND \isin{#2}{left}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[darkmsgdoublecircle, yshift=6.0mm] at (anchor) {#6};
            \node[yshift=2.0mm] at (anchor) {$\leftarrow$};
      }{}

      % doublecircle left arrow down
      \ifthenelse{\isin{#1}{left} \AND \isin{#2}{up}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[darkmsgdoublecircle, xshift=-5.5mm] at (anchor) {#6};
            \node[xshift=-1.5mm] at (anchor) {$\uparrow$};
      }{}
      % doublecircle right arrow down
      \ifthenelse{\isin{#1}{right} \AND \isin{#2}{up}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[darkmsgdoublecircle, xshift=5.5mm] at (anchor) {#6};
            \node[xshift=1.5mm] at (anchor) {$\uparrow$};
      }{}
}
